What Makes Good In-context Demonstrations for Code Intelligence Tasks with LLMs?

Pre-trained models of source code have gained widespread popularity in many code intelligence tasks. Recently, with the scaling of the model and corpus size, large language models have shown the ability of in-context learning (ICL). ICL employs task instructions and a few examples as demonstrations, and then inputs the demonstrations to the language models for making predictions. This new learning paradigm is training-free and has shown impressive performance in various natural language processing and code intelligence tasks. However, the performance of ICL heavily relies on the quality of demonstrations, e.g., the selected examples. It is important to systematically investigate how to construct a good demonstration for code-related tasks. In this paper, we empirically explore the impact of three key factors on the performance of ICL in code intelligence tasks: the selection, order, and number of demonstration examples. We conduct extensive experiments on three code intelligence tasks including code summarization, bug fixing, and program synthesis. Our experimental results demonstrate that all the above three factors dramatically impact the performance of ICL in code intelligence tasks. Additionally, we summarize our findings and provide takeaway suggestions on how to construct effective demonstrations, taking into account these three perspectives. We also show that a carefully-designed demonstration based on our findings can lead to substantial improvements over widely-used demonstration construction methods, e.g., improving BLEU-4, EM, and EM by at least 9.90%, 175.96%, and 50.81% on code summarization, bug fixing, and program synthesis, respectively

==> section/table.tex <==
\begin{table*}[t]
\centering
\caption{RQ1 results on Bug Fixing.}
\aboverulesep=0ex
\belowrulesep=0ex
\scalebox{1}{
\begin{tabular}{lcccc}
\toprule 
\multirow{3}{*}{\textbf{Approach}} &\multicolumn{4}{c}{\textbf{Bug Fixing}}\\ &\multicolumn{2}{c}{\textbf{Small}} &\multicolumn{2}{c}{\textbf{Medium}}\\
\cmidrule{2-5}
& \multicolumn{1}{c}{BLEU-4} & \multicolumn{1}{c}{EM} & BLEU-4 & EM\\
\midrule
& \multicolumn{4}{c}{\textbf{Task-level Demonstration}}\\
\midrule
 {Random$\_$1}  & 72.40 $\pm$ 0.40 &9.52 $\pm$ 1.65 & 87.17 $\pm$ 0.06 &4.35 $\pm$ 2.21\\
 {Random$\_$2}  & 71.09 $\pm$ 0.36 &10.20 $\pm$ 0.15 & 86.77 $\pm$ 0.17 &8.40 $\pm$ 1.30 \\
 {Random$\_$3}  & 70.04 $\pm$ 0.77 &10.13 $\pm$ 0.77 & 86.94 $\pm$ 0.35 &9.03 $\pm$ 0.12 \\
 {Kmeans+Random$\_$1}  & 72.29 $\pm$ 2.17 &8.60 $\pm$ 0.41 & 87.12 $\pm$ 0.04 &8.23 $\pm$ 0.57\\
 {Kmeans+Random$\_$2}  & 71.93 $\pm$ 0.18 &12.78 $\pm$ 0.93 & 86.88 $\pm$ 0.12 &9.61 $\pm$ 0.36\\
 {Kmeans+Random$\_$3}  & 74.44 $\pm$ 1.84 &9.73 $\pm$ 0.38 & 86.72 $\pm$ 0.03 &9.26 $\pm$ 0.86\\
\midrule
& \multicolumn{4}{c}{\textbf{Instance-level Demonstration}}\\
 \midrule
 {BM25}  & 77.54 $\pm$ 0.14 &30.45 $\pm$ 0.4 & 88.05 $\pm$ 0.11 &21.85 $\pm$ 0.50 \\
 {SBERT}  & 76.26 $\pm$ 0.16 &26.15 $\pm$ 0.31 & 87.98 $\pm$ 0.02 &19.00 $\pm$ 0.50\\
 {Unixcoder}  & 77.52 $\pm$ 0.08 &29.93 $\pm$ 0.22 & 87.87 $\pm$ 0.02 &19.14 $\pm$ 0.39\\
 {CoCoSoDa}  & 76.45 $\pm$ 0.08 &27.40 $\pm$ 0.40 & 87.73 $\pm$ 0.07 &19.23 $\pm$ 0.18 \\
\bottomrule
\end{tabular}
}
\end{table*}




\begin{table*}[t]
\centering
\caption{RQ1 results on Program Synthesis and Code Documentation.}\label{tab:RQ1}
\aboverulesep=0ex
\belowrulesep=0ex
\scalebox{0.85}{
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{\textbf{Approach}} & \multicolumn{4}{c}{\textbf{Program Synthesis}} & \multicolumn{3}{c}{\textbf{Code Documentation (CSN)}} & \multicolumn{3}{c}{\textbf{Code Documentation (TLC)}}\\
\cmidrule{2-11}
& \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{SM} & DM & CB & BLEU-4 & ROUGE-L & METEOR & BLEU-4 & ROUGE-L & METEOR \\
\midrule
& \multicolumn{10}{c}{\textbf{Task-level Demonstration}}\\
\midrule
 {Random\_1}  & 16.27 $\pm$ 0.33 &44.73 $\pm$ 0.48 &41.24 $\pm$ 0.95 &28.92 $\pm$ 0.44 & 20.46 $\pm$ 0.53 &36.71 $\pm$ 2.03 &0.0 $\pm$ 0.0 & 16.77 $\pm$ 0.09 &34.62 $\pm$ 0.13 &12.71 $\pm$ 0.01 \\
 {Random\_2}  & 16.20 $\pm$ 0.60 &43.91 $\pm$ 0.55 &39.81 $\pm$ 0.40 &28.43 $\pm$ 0.80 & 19.94 $\pm$ 0.47 &37.17 $\pm$ 0.58 &0.0 $\pm$ 0.0 & 17.94 $\pm$ 0.32 &36.07 $\pm$ 0.31 &12.37 $\pm$ 0.16\\
 {Random\_3}  & 15.53 $\pm$ 0.13 &44.46 $\pm$ 0.45 &37.53 $\pm$ 0.78 &27.72 $\pm$ 0.29  & 18.53 $\pm$ 0.15 &32.50 $\pm$ 0.24 &0.0 $\pm$ 0.0 & 17.15 $\pm$ 0.11 &32.16 $\pm$ 0.41 &12.37 $\pm$ 0.15\\
 {Kmeans+Random\_1}  & 16.87 $\pm$ 0.13 &42.97 $\pm$ 0.07 &37.24 $\pm$ 0.31 &26.64 $\pm$ 0.62 & 20.83 $\pm$ 0.35 &38.42 $\pm$ 0.28 &0.0 $\pm$ 0.0 & 17.81 $\pm$ 0.35 &35.11 $\pm$ 1.38 &0.0 $\pm$ 0.0 \\
 {Kmeans+Random\_2}  & 17.20 $\pm$ 0.40 &45.23 $\pm$ 0.87 &38.60 $\pm$ 2.02 &29.30 $\pm$ 0.98 & 20.62 $\pm$ 0.11 &38.03 $\pm$ 0.19 &0.0 $\pm$ 0.0 &17.88 $\pm$ 0.35 &35.85 $\pm$ 0.63 &0.0 $\pm$ 0.0 \\
 {Kmeans+Random\_3}  & 17.01 $\pm$ 0.21 &44.03 $\pm$ 0.07 &36.09 $\pm$ 0.13 &28.14 $\pm$ 0.14 & 20.67 $\pm$ 0.22 &37.64 $\pm$ 0.20 &0.0 $\pm$ 0.0 & 18.04 $\pm$ 0.17 &36.12 $\pm$ 0.37 &0.0 $\pm$ 0.0\\
\midrule
& \multicolumn{10}{c}{\textbf{Instance-level Demonstration}}\\
 \midrule
 {BM25\_source}  & 18.53 $\pm$ 0.13 &46.22 $\pm$ 0.53 &40.75 $\pm$ 0.58 &30.37 $\pm$ 0.39 & 22.35 $\pm$ 0.14 &38.31 $\pm$ 0.30 &0.0 $\pm$ 0.0 & 36.96 $\pm$ 0.38 &51.42 $\pm$ 0.50 &0.0 $\pm$ 0.0\\
 {SBERT\_source}  & 16.13 $\pm$ 0.53 &44.91 $\pm$ 0.19 &39.81 $\pm$ 1.52 &29.08 $\pm$ 0.25 & 22.27 $\pm$ 0.07 &38.39 $\pm$ 0.22 &0.0 $\pm$ 0.0 & 36.42 $\pm$ 0.29 &50.47 $\pm$ 0.28 &0.0 $\pm$ 0.0\\
 {Unixcoder\_source}  & 16.00 $\pm$ 0.80 &43.93 $\pm$ 0.39 &37.96 $\pm$ 0.60 &28.96 $\pm$ 0.20 & 22.11 $\pm$ 0.17 &38.23 $\pm$ 0.29 &0.0 $\pm$ 0.0 & 36.77 $\pm$ 0.27 &51.11 $\pm$ 0.21 &0.0 $\pm$ 0.0\\
 {CoCoSoDa\_source}  & 16.30 $\pm$ 0.20 &44.62 $\pm$ 0.41 &40.91 $\pm$ 0.59 &29.42 $\pm$ 0.33 & 21.92 $\pm$ 0.14 &37.85 $\pm$ 0.12 &0.0 $\pm$ 0.0 & 36.91 $\pm$ 0.35 &50.69 $\pm$ 0.37 &0.0 $\pm$ 0.0\\
 {SBERT\_target}  & 15.27 $\pm$ 0.53 &44.35 $\pm$ 0.50 &41.62 $\pm$ 1.59 &29.43 $\pm$ 0.65 & 20.24 $\pm$ 0.16 &36.33 $\pm$ 0.23 &0.0 $\pm$ 0.0 & 24.94 $\pm$ 0.23 &40.66 $\pm$ 0.09 &0.0 $\pm$ 0.0\\
 {Unixcoder\_target}  & 18.10 $\pm$ 0.50 &44.53 $\pm$ 0.64 &38.28 $\pm$ 0.46 &28.83 $\pm$ 0.18 & 20.27 $\pm$ 0.10 &36.89 $\pm$ 0.07 &0.0 $\pm$ 0.0 & 25.14 $\pm$ 0.09 &41.62 $\pm$ 0.06 &0.0 $\pm$ 0.0\\
 {CoCoSoDa\_target}  & 18.13 $\pm$ 0.33 &44.88 $\pm$ 0.22 &41.68 $\pm$ 0.61 &30.00 $\pm$ 0.64 & 21.17 $\pm$ 0.12 &36.87 $\pm$ 0.07 &0.0 $\pm$ 0.0 & 27.95 $\pm$ 0.12 &42.73 $\pm$ 0.01 &0.0 $\pm$ 0.0 \\
 {Oracle}  & -- & -- & -- & -- & 27.69 $\pm$ 0.16 &46.17 $\pm$ 0.09 &0.0 $\pm$ 0.0 & 43.16 $\pm$ 0.10 &59.17 $\pm$ 0.07 &0.0 $\pm$ 0.0 \\
\bottomrule
\end{tabular}
}
%\vspace{-0.3cm}
\end{table*}



\begin{table*}[t]
\centering
\caption{Experimental results of different demonstration selection methods on Program Synthesis and Bug Fixing.\gsz{[Since bug fixing is not a bi-modal generation task, we do not apply cross-modality retrieval methods to it. Splitting it into two tables might be better?]} \hy{why some results are '-'}}\label{tab:RQ1B}
\aboverulesep=0ex
\belowrulesep=0ex
\scalebox{0.95}{
\begin{tabular}{l|cccc|cc|cc}
\toprule
\multirow{3}{*}{\textbf{Approach}} & \multicolumn{4}{c|}{\textbf{Program Synthesis}} & \multicolumn{4}{c}{\textbf{Bug Fixing}} \\ 
\cmidrule{2-9}
& \multicolumn{4}{c|}{\textbf{CoNaLa}} & \multicolumn{2}{c|}{\textbf{B2F$_{small}$}} & \multicolumn{2}{c}{\textbf{B2F$_{medium}$}}\\
\cmidrule{2-9}
& \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{SM} & DM & CB & BLEU-4 & EM & BLEU-4 & EM \\
\midrule
& \multicolumn{8}{c}{\textbf{Task-level Demonstration}}\\
\midrule
 {Random\_1}   & 15.53 $\pm$ 0.13 &44.46 $\pm$ 0.45 &37.53 $\pm$ 0.78 &27.72 $\pm$ 0.29  & 72.40 $\pm$ 0.40 &9.52 $\pm$ 1.65 & \textbf{87.17 $\pm$ 0.06} &4.35 $\pm$ 2.21\\
 {Random\_2}  & 16.20 $\pm$ 0.60 &43.91 $\pm$ 0.55 &39.81 $\pm$ 0.40 &28.43 $\pm$ 0.80 & 71.09 $\pm$ 0.36 &10.20 $\pm$ 0.15 & 86.77 $\pm$ 0.17 &8.40 $\pm$ 1.30\\
 {Random\_3}  & 16.27 $\pm$ 0.33 &44.73 $\pm$ 0.48 & \textbf{41.24 $\pm$ 0.95} &28.92 $\pm$ 0.44 & 70.04 $\pm$ 0.77 &10.13 $\pm$ 0.77 & 86.94 $\pm$ 0.35 &9.03 $\pm$ 0.12 \\
 {KRandom\_1}  & 16.87 $\pm$ 0.13 &42.97 $\pm$ 0.07 &37.24 $\pm$ 0.31 &26.64 $\pm$ 0.62 & 72.29 $\pm$ 2.17 &8.60 $\pm$ 0.41 & 87.12 $\pm$ 0.04 &8.23 $\pm$ 0.57\\
 {KRandom\_2}  & \textbf{17.20 $\pm$ 0.40} & \textbf{45.23 $\pm$ 0.87} &38.60 $\pm$ 2.02 & \textbf{29.30 $\pm$ 0.98} & 71.93 $\pm$ 0.18 & \textbf{12.78 $\pm$ 0.93} & 86.88 $\pm$ 0.12 &9.61 $\pm$ 0.36\\
 {KRandom\_3}  & 17.01 $\pm$ 0.21 &44.03 $\pm$ 0.07 &36.09 $\pm$ 0.13 &28.14 $\pm$ 0.14 & \textbf{74.44 $\pm$ 1.84} &9.73 $\pm$ 0.38 & 86.72 $\pm$ 0.03 & \textbf{9.26 $\pm$ 0.86}\\
\midrule
& \multicolumn{8}{c}{\textbf{Instance-level Demonstration}}\\
 \midrule
 {BM-25}  & \textbf{18.53 $\pm$ 0.13} & \textbf{46.22 $\pm$ 0.53} &40.75 $\pm$ 0.58 & \textbf{30.37 $\pm$ 0.39} & \textbf{77.54 $\pm$ 0.14} & \textbf{30.45 $\pm$ 0.40} & \textbf{88.05 $\pm$ 0.11} & \textbf{21.85 $\pm$ 0.50} \\
 {SBERT}  & 16.13 $\pm$ 0.53 &44.91 $\pm$ 0.19 &39.81 $\pm$ 1.52 &29.08 $\pm$ 0.25 & 76.26 $\pm$ 0.16 &26.15 $\pm$ 0.31 & 87.98 $\pm$ 0.02 &19.00 $\pm$ 0.50\\
 {Unixcoder}  & 16.00 $\pm$ 0.80 &43.93 $\pm$ 0.39 &37.96 $\pm$ 0.60 &28.96 $\pm$ 0.20 & 77.52 $\pm$ 0.08 &29.93 $\pm$ 0.22 & 87.87 $\pm$ 0.02 &19.14 $\pm$ 0.39\\
 {CoCoSoDa}  & 16.30 $\pm$ 0.20 &44.62 $\pm$ 0.41 &40.91 $\pm$ 0.59 &29.42 $\pm$ 0.33 & 76.45 $\pm$ 0.08 &27.40 $\pm$ 0.40 & 87.73 $\pm$ 0.07 &19.23 $\pm$ 0.18 \\
 {SBERT$_{cross}$}  & 15.27 $\pm$ 0.53 &44.35 $\pm$ 0.50 & \textbf{41.62 $\pm$ 1.59} &29.43 $\pm$ 0.65 & -- &-- & -- &-- \\
 {Unixcoder$_{cross}$}  & 18.10 $\pm$ 0.50 &44.53 $\pm$ 0.64 &38.28 $\pm$ 0.46 &28.83 $\pm$ 0.18 & -- &-- & -- &--\\ 
 {CoCoSoDa$_{cross}$}  & 18.13 $\pm$ 0.33 &44.88 $\pm$ 0.22 &41.68 $\pm$ 0.61 &30.00 $\pm$ 0.64 & -- &-- & -- &--\\ 
\bottomrule
\end{tabular}
}
%\vspace{-0.3cm}
\end{table*}


\begin{table*}[t]
\centering
\caption{Experimental results of different demonstration selection methods on  Code Summarization.}\label{tab:RQ1_sum}
\aboverulesep=0ex
\belowrulesep=0ex
\scalebox{1}{
\begin{tabular}{l|ccc|ccc}
\toprule 
\multirow{2}{*}{\textbf{Approach}} &\multicolumn{6}{c}{\textbf{Code Summarization}}\\ 
\cmidrule{2-7}
&\multicolumn{3}{c|}{\textbf{CSN}} &\multicolumn{3}{c}{\textbf{TLC}}\\
\cmidrule{2-7}
& BLEU-4 & ROUGE-L & METEOR & BLEU-4 & ROUGE-L & METEOR \\
\midrule
& \multicolumn{6}{c}{\textbf{Task-level Demonstration}}\\
\midrule
 {Random$\_$1}  & 20.46 $\pm$ 0.53 &36.71 $\pm$ 2.03 & 16.17 $\pm$ 0.46 & 16.77 $\pm$ 0.09 &34.62 $\pm$ 0.13 &12.71 $\pm$ 0.01 \\
 {Random$\_$2}  & 19.94 $\pm$ 0.47 &37.17 $\pm$ 0.58 & 16.09 $\pm$ 0.29 & 17.94 $\pm$ 0.32 &36.07 $\pm$ 0.31 &12.37 $\pm$ 0.16\\
 {Random$\_$3}  & 18.53 $\pm$ 0.15 &32.50 $\pm$ 0.24 & 13.63 $\pm$ 0.17 & 17.15 $\pm$ 0.11 &32.16 $\pm$ 0.41 &12.37 $\pm$ 0.15\\
 {KRandom$\_$1}  & \textbf{20.83 $\pm$ 0.35} & \textbf{38.42 $\pm$ 0.28} & \textbf{16.68 $\pm$ 0.16} & 17.81 $\pm$ 0.35 &35.11 $\pm$ 1.38 &12.98 $\pm$ 0.20 \\
 {KRandom$\_$2}  & 20.62 $\pm$ 0.11 &38.03 $\pm$ 0.19 & 16.36 $\pm$ 0.06 &17.88 $\pm$ 0.35 &35.85 $\pm$ 0.63 &13.43 $\pm$ 0.09 \\
 {KRandom$\_$3}  & 20.67 $\pm$ 0.22 &37.64 $\pm$ 0.20 & 15.97 $\pm$ 0.34 & \textbf{18.04 $\pm$ 0.17} & \textbf{36.12 $\pm$ 0.37} & \textbf{14.04 $\pm$ 0.21}\\
\midrule
& \multicolumn{6}{c}{\textbf{Instance-level Demonstration}}\\
 \midrule
 {BM-25}  & \textbf{22.35 $\pm$ 0.14} &38.31 $\pm$ 0.30 & \textbf{17.01 $\pm$ 0.18} & \textbf{36.96 $\pm$ 0.38} & \textbf{51.42 $\pm$ 0.50} & \textbf{24.22 $\pm$ 0.17}\\
 {SBERT}  & 22.27 $\pm$ 0.07 & \textbf{38.39 $\pm$ 0.22} & 16.91 $\pm$ 0.05 & 36.42 $\pm$ 0.29 &50.47 $\pm$ 0.28 &23.86 $\pm$ 0.23\\
 {Unixcoder}  & 22.11 $\pm$ 0.17 &38.23 $\pm$ 0.29 & 16.81 $\pm$ 0.05 & 36.77 $\pm$ 0.27 &51.11 $\pm$ 0.21 &24.08 $\pm$ 0.25\\
 {CoCoSoDa}  & 21.92 $\pm$ 0.14 &37.85 $\pm$ 0.12 & 16.78 $\pm$ 0.06 & 36.91 $\pm$ 0.35 &50.69 $\pm$ 0.37 &24.08 $\pm$ 0.13\\
 {SBERT$_{cross}$}  & 20.24 $\pm$ 0.16 &36.33 $\pm$ 0.23 & 16.00 $\pm$ 0.15 & 24.94 $\pm$ 0.23 &40.66 $\pm$ 0.09 &17.36 $\pm$ 0.14\\
 {Unixcoder$_{cross}$}  & 20.27 $\pm$ 0.10 &36.89 $\pm$ 0.07 & 16.64 $\pm$ 0.06 & 25.14 $\pm$ 0.09 &41.62 $\pm$ 0.06 &17.88 $\pm$ 0.00\\
 {CoCoSoDa$_{cross}$}  & 21.17 $\pm$ 0.12 &36.87 $\pm$ 0.07 & 16.19 $\pm$ 0.07 & 27.95 $\pm$ 0.12 &42.73 $\pm$ 0.01 &18.70 $\pm$ 0.05 \\
 {Oracle  (BM-25)}  & 27.69 $\pm$ 0.16 &46.17 $\pm$ 0.09 & 20.26 $\pm$ 0.06 & 43.16 $\pm$ 0.10 &59.17 $\pm$ 0.07 &28.09 $\pm$ 0.06\\
\bottomrule
\end{tabular}
}
\end{table*}


\begin{table}[t]
\centering
\caption{Experimental results of different demonstration selection methods on Bug Fixing.
}\label{tab:RQ1B}
\aboverulesep=0ex
\belowrulesep=0ex
\scalebox{1}{
\begin{tabular}{l|ccrc|ccrc}
\toprule
\multirow{3}{*}{\textbf{Approach}} & \multicolumn{8}{c}{\textbf{Bug Fixing}} \\ 
\cmidrule{2-9}
& \multicolumn{4}{c|}{\textbf{B2F$_{small}$}} & \multicolumn{4}{c}{\textbf{B2F$_{medium}$}}\\
\cmidrule{2-9}
& \multicolumn{2}{c|}{\textbf{BLEU-4}} & \multicolumn{2}{c|}{\textbf{EM}} & \multicolumn{2}{c|}{\textbf{BLEU-4}} & \multicolumn{2}{c}{\textbf{EM}} \\
& Avg & COV & Avg & COV & Avg & COV & Avg & COV\\
\midrule
& \multicolumn{8}{c}{\textbf{Task-level Demonstration}}\\
\midrule
 {Random}  & 71.18 & 0.25 & 9.95 & 6.02 & \textbf{86.96} & 0.03 & 7.26 & 22.87 \\
 {KmeansRND}  & \textbf{72.89} & 1.87 & \textbf{10.37} & 1.79 & 86.91 & 0.04 & \textbf{9.03} & 2.99\\
\midrule
& \multicolumn{8}{c}{\textbf{Instance-level Demonstration}}\\
 \midrule
 {BM-25}  & \textbf{77.54} & 0.01 & \textbf{30.45} & 0.28 & \textbf{88.05} & 0.01 & \textbf{21.85} & 0.69 \\
 {SBERT}  & 76.26 & 0.02 & 26.15 & 0.20 & 87.98 & 0.00 & 19.00 & 1.56 \\
 {Unixcoder}  & 77.52 & 0.04 & 29.93 & 0.08 & 87.87 & 0.01 & 19.14 & 0.78\\
 {CoCoSoDa}  & 76.45 & 0.05 & 27.40 & 0.30 & 87.73 & 0.00 & 19.23 & 0.11 \\
\bottomrule
\end{tabular}
}
\end{table}



\begin{table}[t]
\centering
\caption{Experimental results of different demonstration selection methods on Program Synthesis.}\label{tab:RQ1p}
\aboverulesep=0ex
\belowrulesep=0ex
\scalebox{0.85}{
\begin{tabular}{l|cccccccc}
\toprule
\multirow{2}{*}{\textbf{Approach}} & \multicolumn{8}{c}{\textbf{Program Synthesis}} \\
\cmidrule{2-9}
& \multicolumn{2}{c|}{EM} & \multicolumn{2}{c|}{SM} & \multicolumn{2}{c|}{DM} & \multicolumn{2}{c}{CB} \\
& Avg & COV & Avg & COV & Avg & COV & Avg & COV\\
\midrule
& \multicolumn{8}{c}{\textbf{Task-level Demonstration}}\\
\midrule
 {Random}  & 16.00 & 0.53 & 44.37 & 0.31 & \textbf{39.70} & 0.77 & \textbf{28.36} & 0.55\\
 {KmeansRND}  & \textbf{17.03} & 0.23  & \textbf{44.41} & 0.29  & 37.31 & 1.82  & 28.03 & 0.82  \\
\midrule
& \multicolumn{8}{c}{\textbf{Instance-level Demonstration}}\\
 \midrule
 {BM-25}  & \textbf{18.53} & 0.05 & \textbf{46.22} & 0.33 & 40.75 & 0.46 & \textbf{30.37} & 0.26 \\
 {SBERT}  & 16.13 & 1.05 &44.91& 0.04 & 39.81 & 3.61 & 29.08 & 0.14 \\
 {Unixcoder}  & 16.00 & 2.00 & 43.93 & 0.20 & 37.96 & 0.48 & 28.96 & 0.07 \\
 {CoCoSoDa}  & 16.30 & 0.12 & 44.62 & 0.22 & 40.91 & 0.52 & 29.42 & 0.20 \\
 {SBERT$_{cross}$}  & 15.27 & 0.93 & 44.35 & 0.29 & 41.62 & 3.53 & 29.43& 0.75 \\
 {Unixcoder$_{cross}$}  & 18.10& 0.70  & 44.53 & 0.59 & 38.28 & 0.33 & 28.83 & 0.06 \\ 
 {CoCoSoDa$_{cross}$}  & 18.13 & 0.34 & 44.88 & 0.05 & \textbf{41.68} & 0.47 & 30.00 & 0.88 \\ 
\bottomrule
\end{tabular}
}8
\end{table}




\begin{table*}[t]
\centering
\caption{Experimental results of different demonstration selection methods on  Code Summarization.}\label{tab:RQ1_sum}
\aboverulesep=0ex
\belowrulesep=0ex
\scalebox{1}{
\begin{tabular}{l|cccccc|cccccc}
\toprule 
\multirow{2}{*}{\textbf{Approach}} &\multicolumn{12}{c}{\textbf{Code Summarization}}\\ 
\cmidrule{2-13}
&\multicolumn{6}{c|}{\textbf{CSN}} &\multicolumn{6}{c}{\textbf{TLC}}\\
\cmidrule{2-13}
& \multicolumn{2}{c}{\textbf{BLEU-4}} & \multicolumn{2}{c}{\textbf{ROUGE-L}} & \multicolumn{2}{c}{\textbf{METEOR}} & \multicolumn{2}{c}{\textbf{BLEU-4}} & \multicolumn{2}{c}{\textbf{ROUGE-L}} & \multicolumn{2}{c}{\textbf{METEOR}}\\
& Avg & COV & Avg & COV & Avg & COV & Avg & COV & Avg & COV & Avg & COV\\
\midrule
& \multicolumn{12}{c}{\textbf{Task-level Demonstration}}\\
\midrule
 {Random}  & 19.64 & 0.50 & 35.46 & 2.09 & 12.30 & 0.43 & 17.29 & 0.12 & 34.28 & 0.15 &12.48 & 0.08 \\
 {KmeansRND}  & \textbf{20.71} & 0.16 & \textbf{38.03} & 0.07 & \textbf{16.34} & 0.16 & \textbf{17.91} & 0.27 & \textbf{35.69} & 1.17 & \textbf{13.48} & 0.13 \\
\midrule
& \multicolumn{12}{c}{\textbf{Instance-level Demonstration}}\\
 \midrule
 {BM-25}  & \textbf{22.35} & 0.05 &38.31 & 0.12 & \textbf{17.01} & 0.10 & \textbf{36.96} & 0.27 & \textbf{51.42} & 0.32 & \textbf{24.22} & 0.24\\
 {SBERT}  & 22.27 & 0.01 & \textbf{38.39} & 0.07 & 16.91 & 0.08 & 36.42 & 0.14 &50.47 & 0.08 &23.86 & 0.11\\
 {Unixcoder}  & 22.11 & 0.08 &38.23 & 0.11 & 16.81 & 0.09 & 36.77 & 0.10 &51.11 & 0.04 &24.08 & 0.15\\
 {CoCoSoDa}  & 21.92 & 0.05 &37.85 & 0.02 & 16.78 & 0.01 & 36.91 & 0.18 &50.69 & 0.15 &24.08 & 0.04\\
 {SBERT$_{cross}$}  & 20.24 & 0.07 &36.33 & 0.07 & 16.00 & 0.08 & 24.94 & 0.17 &40.66 & 0.08 &17.36 & 0.10\\
 {Unixcoder$_{cross}$}  & 20.27 & 0.03 &36.89 & 0.01 & 16.64 & 0.04 & 25.14 & 0.02 &41.62 & 0.01 &17.88\ & 0.00\
 {CoCoSoDa$_{cross}$}  & 21.17 & 0.03 &36.87 & 0.01 & 16.19 & 0.01 & 27.95 & 0.12 &42.73 & 0.02 &18.70 & 0.02\\
 {Oracle  (BM-25)}  & 27.69 & 0.05 &46.17 & 0.01 & 20.26 & 0.01 & 43.16 & 0.01 &59.17 & 0.00 &28.09 & 0.01\\
\bottomrule
\end{tabular}
}
\end{table*}


\begin{table}[t]
    \centering
    \caption{Experiments of generalization on other LLMs. Avg, VarO, and VarE denote the average results, the variance of different orders and the variance of different groups of examples, respectively.}
\aboverulesep=0ex
\belowrulesep=0ex
 \scalebox{0.95}{
    \begin{tabular}{c|rrrrrr}
    \toprule
    \multicolumn{1}{c|}{{\multirow{2}{*}{\textbf{Approach}}}} & \multicolumn{3}{c}{\textbf{EM}} & \multicolumn{3}{c}{\textbf{CB}}  \\
    \cmidrule{2-7} 
    & Avg & VarO & VarE & Avg & VarO & VarE \\
    \midrule
    & \multicolumn{6}{c}{GPT-3.5} \\ 
    \midrule
    \multicolumn{1}{l|}{Random+Random} & 12.32 & 1.32 & 0.93 & 26.60 & 0.41 & 0.67 \\
    \multicolumn{1}{l|}{KmeansRND+Random}  & 13.60 & 0.41 & 0.66 & 28.26 & 0.02 & 0.20 \\
    \multicolumn{1}{l|}{Unixcoder+Random}  & 13.73 & 0.25 & -- & 30.06 & 0.31 & -- \\
    \multicolumn{1}{l|}{BM-25+Random} & 14.40 & 0.16 & -- & 30.81 & 0.15 & --  \\
    \multicolumn{1}{l|}{BM-25+Similarity}  & 15.20 & -- & -- & 30.69 & -- & -- \\
    \midrule
    & \multicolumn{6}{c}{ChatGPT} \\ 
    \midrule
    \multicolumn{1}{l|}{Random+Random} & 11.88 & 0.49 & 1.15 & 28.17 & 0.71 & 0.43 \\
    \multicolumn{1}{l|}{KmeansRND+Random}  & 12.92 & 0.09 & 0.37 & 28.25 & 1.15 & 0.19 \\
    \multicolumn{1}{l|}{Unixcoder+Random}  & 14.32 & 1.01 & -- & 29.33 & 0.43 & -- \\
    \multicolumn{1}{l|}{BM-25+Random} & 13.47 & 0.09 & -- & 28.95 & 1.04 & --  \\
    \multicolumn{1}{l|}{BM-25+Similarity}  & 14.20 & -- & -- & 30.03 & -- & -- \\
    \bottomrule
    \end{tabular}
    \label{tab:generalization}}
\end{table}




\begin{table}[t]
\centering
\caption{periments of generalization on GPT3.5 and ChatGPT. Avg and CV denote the average results and Coefficient of Variation over three different orders, respectively.}\label{tab:generalization}
\aboverulesep=0ex
\belowrulesep=0ex
\scalebox{1}{
\begin{tabular}{l|cccc}
\toprule
\multirow{3}{*}{\textbf{Approach}} & \multicolumn{4}{c}{\textbf{Program Synthesis}} \\
\cmidrule{2-5}
& \multicolumn{2}{c}{CB} & \multicolumn{2}{c}{EM} \\
& Avg & CV & Avg & CV\\
\midrule
& \multicolumn{4}{c}{\textbf{GPT-3.5}}\\
\midrule
 {Random+Random}  & 26.60 & 4.50 & 12.32 & 4.30 \\
 {KmeansRND+Random}  & 28.26 & 1.76  & 13.60 & 0.58 \\
 {Unixcoder+Random}  & 30.06 & 0.34 & 13.73 & 0.45 \\
 {BM-25+Random}  & 30.81 & 0.09  & 14.40 & 0.19 \\
 {BM-25+Similarity}  & 30.69 & 0.00  & 15.20 &  0.00 \\
\midrule
& \multicolumn{4}{c}{\textbf{ChatGPT}}\\
 \midrule
 {Random+Random}  & 28.17 & 1.12 & 11.88 & 2.20 \\
 {KmeansRND+Random}  & 28.25 & 1.65  & 12.92 & 0.43 \\
 {Unixcoder+Random}  & 29.33 & 0.97 & 14.32 & 4.74 \\
 {BM-25+Random}  & 28.95 & 2.39  & 13.47 & 0.46 \\
 {BM-25+Similarity}  & 30.03 & 0.00   & 14.20 & 0.00  \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table*}[t]
    \centering
    \caption{Comparison of %supervised state-of-the-art methods and
    different demonstration construction methods on three LLMs. %The results of code summariation, bug fixing, and program synthesis are taken from CodeT5~\cite{DBLP:conf/emnlp/0034WJH21}, NatGen~\cite{DBLP:conf/sigsoft/ChakrabortyADDR22} and CodePAD~\cite{DBLP:journals/corr/abs-2211-00818} respectively\hy{which results for which model? (CodeT5, NatGen, CodePad}
    }
\aboverulesep=0ex
\belowrulesep=0ex
 \scalebox{1}{
    \begin{tabular}{c|ccc|cc|cccc}
    \toprule
    \multicolumn{1}{c|}{{\multirow{2}{*}{\textbf{Approach}}}} & \multicolumn{3}{c|}{Code Summarization (CSN)} & \multicolumn{2}{c|}{Bug Fixing (B2F$_{small}$)} & \multicolumn{4}{c}{Program Synthesis (CoNaLa)} \\
    \cmidrule{2-10} 
    &BLEU-4 & ROUGE-L & METEOR  &  BLEU-4 & EM & CB & SM & DM & EM  \\
    \midrule
    %\multicolumn{1}{l|}{Supervised model} & 20.31 & -- & -- & -- & 23.43 & 3.5 & -- & -- & --\\
    % \midrule
    % \multicolumn{1}{l}{} & \multicolumn{9}{c}{Code-davinci-002} \\
    % \midrule
    % \multicolumn{1}{l|}{Zero-shot} & 1.82 & 4.27 & 4.19 & 34.65 & 1.43 & 0.20 & 9.26 & 23.81 & 8.71 \\
    % \multicolumn{1}{l|}{Simple demonstration}  & 18.68 & 32.74 & 13.80 & 69.39 & 9.75 & 15.60 & 44.91 & 36.84 & 28.01 \\
    % \multicolumn{1}{l|}{Well-designed demonstration} & \textbf{22.73} & 39.52 & 17.35 & 77.54 & \textbf{32.07} & \textbf{21.40} & 48.03 & 42.88 & 32.25 \\
    %\midrule
    \multicolumn{1}{l}{} & \multicolumn{9}{c}{Codex} \\
    \midrule
    \multicolumn{1}{c|}{Zero-shot} & 1.82 & 4.27 & 4.19 & 34.65 & 1.43 & 8.71 & 9.26 & 23.81 & 0.20 \\
    \multicolumn{1}{c|}{Baseline demonstration}  & 17.37 & 32.04 & 13.43 & 69.07 & 9.70 & 27.54 & 44.56 & 37.07 & 14.20 \\
    \multicolumn{1}{c|}{Carefully-designed demonstration} & \textbf{22.73} & \textbf{39.52} & \textbf{17.35} & \textbf{77.54}  & \textbf{32.25}  & \textbf{32.07} & \textbf{48.03} & \textbf{42.88}  & \textbf{21.40}\\
    \midrule
    \multicolumn{1}{l}{} & \multicolumn{9}{c}{GPT-3.5} \\
    \midrule
    \multicolumn{1}{c|}{Zero-shot} & 6.34 & 15.05 & 14.08 & 2.81 & 0.15 & 0.06& 0.26 & 0.00  & 0.20 \\
    \multicolumn{1}{c|}{Baseline demonstration}  & 14.55 & 21.53 & 13.81 & 62.87 & 9.15 & 26.36 & 36.94 & 41.67 & 10.00 \\
    \multicolumn{1}{c|}{Carefully-designed demonstration} & \textbf{15.99} & \textbf{26.78} & \textbf{16.70} & \textbf{71.70} & \textbf{25.25} & \textbf{30.69}  & \textbf{43.95} & \textbf{44.78} & \textbf{15.20} \\
    \midrule
    \multicolumn{1}{l}{} & \multicolumn{9}{c}{ChatGPT} \\
    \midrule
    \multicolumn{1}{c|}{Zero-shot} & 3.63 & 11.40 & 13.16 & 2.32 & 0.05 & 25.70 & 37.64 & 54.44 & 3.40 \\
    \multicolumn{1}{c|}{Baseline demonstration}  & 10.76 & 20.02 & 14.83 & 41.57 & 4.60 & 27.62 & 41.83 & 46.85 & 9.40 \\
    \multicolumn{1}{c|}{Carefully-designed demonstration} & \textbf{11.90} & \textbf{23.31} & \textbf{16.93} & \textbf{53.92} & \textbf{18.15} & \textbf{30.03} & \textbf{45.04} & \textbf{44.26} & \textbf{14.20} \\
    \bottomrule
    \end{tabular}
    \label{tab:comparison}}
\end{table*}


\begin{table*}[t]
    \centering
    \caption{Comparison of different demonstration construction methods on three LLMs.}
\aboverulesep=0ex
\belowrulesep=0ex
 \scalebox{1}{
    \begin{tabular}{cc|rrr|rr|rrrr}
    \toprule
    \multicolumn{2}{c|}{{\multirow{2}{*}{\textbf{Approach}}}} & \multicolumn{3}{c|}{Code Summarization (CSN)} & \multicolumn{2}{c|}{Bug Fix (B2F$_{small}$)} & \multicolumn{4}{c}{Program Synthesis (CoNaLa)} \\
    \cmidrule{3-11} 
     &  &BLEU-4 & ROUGE-L & METEOR  & BLEU-4 & EM & \multicolumn{1}{c}{CB} & \multicolumn{1}{c}{SM} & DM & EM  \\
    \midrule
    \multirow{3}{*}{Codex} & \multicolumn{1}{c|}{Zero-shot} & 1.82 & 4.27 & 4.19 & 34.65 & 1.43 & 8.71 & 9.26 & 23.81 & 0.20 \\
    \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{Baseline demonstration}  & 17.37 & 32.04 & 13.43 & 69.07 & 9.70 & 27.54 & 44.56 & 37.07 & 14.20 \\
    \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{Carefully-designed demonstration} & \textbf{22.73} & \textbf{39.52} & \textbf{17.35} & \textbf{77.54}  & \textbf{32.25}  & \textbf{32.07} & \textbf{48.03} & \textbf{42.88}  & \textbf{21.40} \\
    \midrule
    \multirow{3}{*}{GPT-3.5} & \multicolumn{1}{c|}{Zero-shot} & 6.34 & 15.05 & 14.08 & 2.81 & 0.15 & 0.06& 0.26 & 0.00  & 0.20 \\
    \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{Baseline demonstration}  & 14.55 & 21.53 & 13.81 & 62.87 & 9.15 & 26.36 & 36.94 & 41.67 & 10.00 \\
    \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{Carefully-designed demonstration} & \textbf{15.99} & \textbf{26.78} & \textbf{16.70} & \textbf{71.70} & \textbf{25.25} & \textbf{30.69}  & \textbf{43.95} & \textbf{44.78} & \textbf{15.20} \\
    \midrule
    \multirow{3}{*}{ChatGPT} &\multicolumn{1}{c|}{Zero-shot} & 3.63 & 11.40 & 13.16 & 2.32 & 0.05 & 25.70 & 37.64 & 54.44 & 3.40 \\
    \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{Baseline demonstration}  & 10.76 & 20.02 & 14.83 & 41.57 & 4.60 & 27.62 & 41.83 & 46.85 & 9.40 \\
    \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{Carefully-designed demonstration} & \textbf{11.90} & \textbf{23.31} & \textbf{16.93} & \textbf{53.92} & \textbf{18.15} & \textbf{30.03} & \textbf{45.04} & \textbf{44.26} & \textbf{14.20} \\
    \bottomrule
    \end{tabular}
    \label{tab:comparison}}
\end{table*}
